A regularized tri-linear approach for optical interferometric imaging

In the context of optical interferometry, only undersampled power spectrum and bispectrum data are accessible. It poses an ill-posed inverse problem for image recovery. Recently, a tri-linear model was proposed for monochromatic imaging, leading to an alternated minimization problem. In that work, only a positivity constraint was considered, and the problem was solved by an approximated Gauss-Seidel method. In this paper, we propose to improve the approach on three fundamental aspects. Firstly, we define the estimated image as a solution of a regularized minimization problem, promoting sparsity in a fixed dictionary using either an $\ell_1$ or a weighted-$\ell_1$ regularization term. Secondly, we solve the resultant non-convex minimization problem using a block-coordinate forward-backward algorithm. This algorithm is able to deal both with smooth and non-smooth functions, and benefits from convergence guarantees even in a non-convex context. Finally, we generalize our model and algorithm to the hyperspectral case, promoting a joint sparsity prior through an $\ell_{2,1}$ regularization term. We present simulation results, both for monochromatic and hyperspectral cases, to validate the proposed approach.

==> intro.tex <==


With the advent of astronomical interferometers, it has become possible to image the sky at very high angular resolution.
An interferometer basically consists of an array of telescopes such that each pair of telescopes probes a spatial frequency in the Fourier plane (denoted by $u-v$ plane) of the image of interest. Given the limited number of telescopes, incomplete sampling of the $u-v$ plane is obtained. 
In particular, for radio interferometry, measurements consist of complex visibilities, related to Fourier coefficients of the intensity image of interest \citep{Thompson2001}. In this context, the incomplete Fourier sampling leads to a linear ill-posed inverse problem for image reconstruction, and iterative algorithms need to be designed to solve this problem. 
Classical reconstruction methods for radio interferometry are mainly based on iterative deconvolution (\textsc{clean}; \cite{Hogbom1974}), and on {maximum entropy methods} (MEM) to impose smoothness on the sought image by maximizing the entropy of the image \citep{Cornwell1985}. More recently, imaging techniques within the framework of compressive sensing have been proposed  \citep{Wiaux2009}. 
These methods rely on finding an image that is sparse in a given dictionary, using convex optimization algorithms \citep{Boyd2004, Combettes2010}. 

As compared to the radio interferometers, optical interferometers involve a less number of telescopes, which in turn provides a sparser $u-v$ coverage. Moreover, atmospheric turbulence at optical wavelengths causes random phase fluctuations leading to cancellation of the visibility values. Indeed the measurements consist of phase insensitive observables: power spectrum and bispectrum, resulting into loss of partial phase information \citep{Thiebaut2010}. 
This induces non-linearity in the inverse problem for image reconstruction in optical interferometry. Thus, the image recovery methods used in radio interferometry cannot be directly applied, and new methods need to be developed.

Research in this direction has led to the development of various algorithms, based on different approaches. In \citet{Thiebaut2008}, the so-called MIRA method has been developed, using a {maximum a posteriori} (MAP) approach to recover the image, where different types of quadratic regularization can be considered. 
The author proposed to solve the resulting minimization problem using
a limited variable metric algorithm which accounts for parameter bounds (namely, the VMLMB algorithm \citep{Thiebaut2002}).  
Another technique, proposed by \citet{Meimon2005}, namely WISARD, makes use of a self-calibration approach to solve for missing phase information, using smooth regularizations. 
The so-called BSMEM method, proposed in \citet{Buscher1994}, consists of using MEM to impose smoothness on the estimated image. Recently, \citet{Hofmann2014} proposed the IRBis method (image reconstruction software using the bispectrum), which solves the minimization problem from a MAP approach, considering smooth regularization terms, and employing a non-linear optimization algorithm based on conjugate gradients \citep{Hager2005,Hager2006a}. 
However, due to the non-linearity of the considered inverse problem, the minimization problems solved by the above methods perform only local optimization. 
For global minimum search, different approaches have been proposed these last years. In particular, techniques based on a {Markov Chain Monte Carlo} (MCMC) method \citep{Gamerman1997} have been adopted in MACIM \citep{Ireland2006a} and SQUEEZE \citep{Baron2012}, while in \citet{Auria2013}, a tensor approach has been proposed. 
In the latter, following the idea of phase-lift methods for phase retrieval problems \citep{Cand2011, Waldspurger2013}, the data model is lifted from a vector to a super-symmetric rank-1 order-3 tensor formed by the tensor product of the vector representing the sought image with itself. This yields a linear inverse problem, and a convex minimization problem can be deduced from a MAP approach. In \citet{Auria2014}, the tensor approach has been extended to account for the signal sparsity and thereby improving the reconstruction quality. However, solving for order-3 tensor  instead of an image (i.e. a vector) increases the dimensionality of the problem drastically and makes this approach computationally very expensive. 
Thus, \citet{Auria2013} proposed another method which involves solving linear and convex sub-problems alternately and iteratively for 3 images. 
Although the global minimization problem remains non-convex and dependent on the initial guess, in practice it has been shown that it provides much better reconstruction quality and accelerates the convergence speed as compared to the tensor approach. 
Moreover, contrary to the state-of-the-art-methods, it brings convexity to the sub-problems. 
However, \citet{Auria2013} proposed to solve the tri-linear problem using a Gauss-Seidel method {(\citet{Zangwill1969}, \citet[Chap~7]{Ortega1970}, \citet[Chap.2]{Bertsekas1999})}, which does not have any convergence guarantees in this context. Additionally, only positivity constraints have been considered, without imposing any other \emph{a priori} information on the underlying image. 


All of the above mentioned methods are designed to reconstruct monochromatic images. 
However, electromagnetic radiations at different wavelengths can be emitted from an astrophysical source, corresponding to its spectrum.
In order to exploit the spectrum of the source, modern optical interferometers are paving the way for multi-wavelength imaging. Instruments such as AMBER \citep{Petrov2001}, GRAVITY \citep{Eisenhauer2008} and MATISSE \citep{Lopez2009}, can take measurements at multiple wavelength channels. 
This necessitates the progression of imaging techniques from monochromatic to hyperspectral case. 
Lately, initial work are done in the direction of hyperspectral imaging for optical interferometry. 
In particular, the method proposed by \citet{Kluska2014}, namely SPARCO, is a semi-parametric approach for image reconstruction of chromatic objects, whereas the method proposed by \citet{Thiebaut2013} deals with a sparsity regularized approach considering the observed scene to be a collection of point-like sources. Recently the use of differential phases for hyperspectral imaging has been proposed in PAINTER \citep{Schutz2014}. The methods proposed by \citet{Thiebaut2013} and \citet{Schutz2014} use the {alternating direction method of multipliers} (ADMM) algorithm \citep{Boyd2010} to solve the considered minimization problem. 

In this article, we propose an image reconstruction algorithm which can be applied both for monochromatic and hyperspectral cases in optical interferometry. 
More precisely, in the monochromatic case, we propose to improve the method based on the tri-linear data model proposed by \citet{Auria2013}.
First, we propose to impose sparsity as a regularization term, by means of an $\ell_1$-norm, either in the image domain or in a given basis \citep{Wiaux2009, Carrillo2012}, leveraging the recent compressive sensing theory \citep{Donoho2006}. 
In addition, we have developed an algorithm, based on the block-coordinate forward-backward algorithm recently proposed, e.g., by \citet{Bolte2014,Frankel2015,Chouzenoux2016}, which allows to deal with non-necessarily smooth regularization terms such as the $\ell_1$ norm. Moreover, this algorithm benefits from the convergence guarantees even for the non-convex global minimization problems. 
Finally, we generalize the proposed method to the hyperspectral case. It translates to a new approach for hyperspectral imaging in optical interferometry. We exploit the joint sparsity of the image cube through an $\ell_{2,1}$ norm \citep{Thiebaut2013}.

The rest of the article is organized as follows. Section~\ref{sec:optical_imaging} describes the observation model, whereas the corresponding regularized minimization problem is detailed in Section~\ref{sec:min_prob}. In Section~\ref{sec:proposed_algo}, the proposed algorithm to solve the resultant minimization problem is presented along with the implementation details, incorporating various regularization terms. The simulations performed and the results obtained thereby for monochromatic case are discussed in Section~\ref{sec:simulations}.  Section~\ref{sec:hyperspectral} is devoted to the hyperspectral case. Starting with the problem statement, the optimization details and the simulations performed are then presented with the results obtained. Finally, the conclusion is provided in Section~\ref{sec:Conclusion}.

